Rumor Mitigation in Social Media Platforms with Deep Reinforcement Learning

Social media platforms have become one of the main channels where people disseminate and acquire information, of which the reliability is severely threatened by rumors widespread in the network. Existing approaches such as suspending users or broadcasting real information to combat rumors are either with high cost or disturbing users. In this paper, we introduce a novel rumor mitigation paradigm, where only a minimal set of links in the social network are intervened to decelerate the propagation of rumors, countering misinformation with low business cost and user awareness. A knowledge-informed agent embodying rumor propagation mechanisms is developed, which intervenes the social network with a graph neural network for capturing information flow in the social media platforms and a policy network for selecting links. Experiments on real social media platforms demonstrate that the proposed approach can effectively alleviate the influence of rumors, substantially reducing the affected populations by over 25%. Codes for this paper are released at https://github.com/tsinghua-fib-lab/DRL-Rumor-Mitigation.

==> related.tex <==
\section{Related Work}
\begin{table}[t]
\caption{
Rumor mitigation performance when transferring directly to larger social networks.
For example, TS2TM donates that the model trained with Twitter S is directly used for Twitter M, and the others are similar.
Higher is better.}
\vspace{-5px}
\label{tab::transfer}
\begin{tabular}{c|c|c|c|c|c}
\toprule

Strategy & TS2TM & TS2TL & TM2TL & TS2FL & TM2FL \\
\midrule
from scratch & 31.32 & 32.18 & 32.18 & 37.26 & 37.26  \\
transfer & 27.96 & $ $27.13$ $ & $ $30.19$ $ & 28.56 & 32.36 \\
DRLN & 26.16 & 26.81 & 26.81 & 29.67 & 29.67  \\

\bottomrule
\end{tabular}
\vspace{-5px}
\end{table}


\noindent\textbf{Deep Reinforcement Learning on Graph.}
The integration of DRL with graph-structureed data is a rapidly advancing field.
Leveraging the powerful representation learning capabilities of GNN~\cite{kipf2016semi}, DRL methods have achieved success across diverse domains, such as recommendation systems~\cite{ma2023sgnr,guo2022reinforcement,chen2023trip}, drug discovery~\cite{mcnaughton2022novo,knutson2022decoding,do2019graph}, traffic management~\cite{almasan2022deep,jin2018hierarchical,yang2021ihg}, and chip design~\cite{wang2020gcn,myung2021policy,zhu2020exploring}.
Deep learning techniques~\cite{lecun2015deep} can 
handle high-demensional inputs, allowing for the learning of comprehensive embeddings that capture complex relationships and interactions within graph-structured data.
On the other hand, organizing data in a graphical format provides the agent richer information, leading to a helpful decision-making.
In this study, we conceptualize the task of rumor mitigation as a sequential edge selection problem within a graph framework. 
To the best of our knowledge, we pioneer the application of DRL and GNN to address this problem for the first time.


\noindent\textbf{Rumor Mitigation on Social Media Platforms.}
As an extensively studied issue~\cite{meel2020fake,sharma2019combating,saxena2022fake}, rumor mitigation methods can be divided into two primary categories: influence blocking and anti-rumor propagation.
The influence blocking method stops the spread of rumors by isolating key nodes or edges in the network.
Heuristic method~\cite{holme2002attack,gao2011network,comin2011identifying,dey2017centrality,preciado2014optimal,yang2021targeted,kitsak2010identification,wang2013negative,amoruso2020contrasting} is a popular approach to recognize important elements on the network based on topological features like degree~\cite{holme2002attack,gao2011network} and betweenness~\cite{comin2011identifying,dey2017centrality}.
However, they can not fully sense the network structure and tend to be ineffective in mitigating the spread of misinformation.
Greedy method~\cite{wu2019minimizing,pham2018targeted,yang2019influence} is another powerful approach with $(1-1/e)$-approximation~\cite{kempe2003maximizing}, which explores all candidates and select the one with the minimum rumor impact at each step.
Recent researches~\cite{he2022reinforcement,meirom2021controlling} formulate the rumor mitigation task as a MDP on the graph and apply RL algorithm to solve it.
However, they mainly focus on blocking users, which is an expensive and coarse control for rumors, and lacks a design for the characteristics of rumor spreading.
Anti-rumor propagation is also feasible for rumor mitigation~\cite{garrett2009echo,van2017inoculating,cook2017neutralizing}, which reduces the propagation of rumor by informing users the truth and competing with rumor in the social media platforms.
Similar to the influence blocking method, heuristic~\cite{xu2010toward,tong2018misinformation}, greedy~\cite{taninmics2020minimizing,nguyen2012containment,budak2011limiting} and machine learning ~\cite{farajtabar2017fake,he2022graph} approaches are also applied for anti-rumor propagation.
Nevertheless, combating rumors relies on deep user engagement, making anti-rumor propagation expensive and hard to control.
Different from existing works, we propose an innovative framework for rumor mitigation, where a minimal set of edges are intelligently blocked by a DRL agent, with knowledge-informed model design fully capturing the rumor propagation mechanisms.





































